Real-Time Evaluation in Online Continual Learning: A New Hope

Current evaluations of Continual Learning (CL) methods typically assume that there is no constraint on training time and computation. This is an unrealistic assumption for any real-world setting, which motivates us to propose: a practical real-time evaluation of continual learning, in which the stream does not wait for the model to complete training before revealing the next data for predictions. To do this, we evaluate current CL methods with respect to their computational costs. We conduct extensive experiments on CLOC, a large-scale dataset containing 39 million time-stamped images with geolocation labels. We show that a simple baseline outperforms state-of-the-art CL methods under this evaluation, questioning the applicability of existing methods in realistic settings. In addition, we explore various CL components commonly used in the literature, including memory sampling strategies and regularization approaches. We find that all considered methods fail to be competitive against our simple baseline. This surprisingly suggests that the majority of existing CL literature is tailored to a specific class of streams that is not practical. We hope that the evaluation we provide will be the first step towards a paradigm shift to consider the computational cost in the development of online continual learning methods.

==> egdbib_old <==
@String(PAMI = {IEEE Trans. Pattern Anal. Mach. Intell.})
@String(IJCV = {Int. J. Comput. Vis.})
@String(CVPR= {IEEE Conf. Comput. Vis. Pattern Recog.})
@String(ICCV= {Int. Conf. Comput. Vis.})
@String(ECCV= {Eur. Conf. Comput. Vis.})
@String(NIPS= {Adv. Neural Inform. Process. Syst.})
@String(ICPR = {Int. Conf. Pattern Recog.})
@String(BMVC= {Brit. Mach. Vis. Conf.})
@String(TOG= {ACM Trans. Graph.})
@String(TIP  = {IEEE Trans. Image Process.})
@String(TVCG  = {IEEE Trans. Vis. Comput. Graph.})
@String(TMM  = {IEEE Trans. Multimedia})
@String(ACMMM= {ACM Int. Conf. Multimedia})
@String(ICME = {Int. Conf. Multimedia and Expo})
@String(ICASSP=	{ICASSP})
@String(ICIP = {IEEE Int. Conf. Image Process.})
@String(ACCV  = {ACCV})
@String(ICLR = {Int. Conf. Learn. Represent.})
@String(IJCAI = {IJCAI})
@String(PR   = {Pattern Recognition})
@String(AAAI = {AAAI})
@String(CVPRW= {IEEE Conf. Comput. Vis. Pattern Recog. Worksh.})
@String(CSVT = {IEEE Trans. Circuit Syst. Video Technol.})

@String(SPL	= {IEEE Sign. Process. Letters})
@String(VR   = {Vis. Res.})
@String(JOV	 = {J. Vis.})
@String(TVC  = {The Vis. Comput.})
@String(JCST  = {J. Comput. Sci. Tech.})
@String(CGF  = {Comput. Graph. Forum})
@String(CVM = {Computational Visual Media})


@String(PAMI  = {IEEE TPAMI})
@String(IJCV  = {IJCV})
@String(CVPR  = {CVPR})
@String(ICCV  = {ICCV})
@String(ECCV  = {ECCV})
@String(NIPS  = {NeurIPS})
@String(ICPR  = {ICPR})
@String(BMVC  =	{BMVC})
@String(TOG   = {ACM TOG})
@String(TIP   = {IEEE TIP})
@String(TVCG  = {IEEE TVCG})
@String(TCSVT = {IEEE TCSVT})
@String(TMM   =	{IEEE TMM})
@String(ACMMM = {ACM MM})
@String(ICME  =	{ICME})
@String(ICASSP=	{ICASSP})
@String(ICIP  = {ICIP})
@String(ACCV  = {ACCV})
@String(ICLR  = {ICLR})
@String(IJCAI = {IJCAI})
@String(PR = {PR})
@String(AAAI = {AAAI})
@String(CVPRW= {CVPRW})
@String(CSVT = {IEEE TCSVT})


@article{McCloskey1989,
   abstract = {Connectionist networks in which information is stored in weights on connections among simple processing units have attracted considerable interest in cognitive science. Much of the interest centers around two characteristics of these networks. First, the weights on connections between units need not be prewired by the model builder but rather may be established through training in which items to be learned are presented repeatedly to the network and the connection weights are adjusted in small increments according to a learning algorithm. Second, the networks may represent information in a distributed fashion. This chapter discusses the catastrophic interference in connectionist networks. Distributed representations established through the application of learning algorithms have several properties that are claimed to be desirable from the standpoint of modeling human cognition. These properties include content-addressable memory and so-called automatic generalization in which a network trained on a set of items responds correctly to other untrained items within the same domain. New learning may interfere catastrophically with old learning when networks are trained sequentially. The analysis of the causes of interference implies that at least some interference will occur whenever new learning may alter weights involved in representing old learning, and the simulation results demonstrate only that interference is catastrophic in some specific networks. © 1989 Academic Press Inc.},
   author = {Michael McCloskey and Neal J. Cohen},
   doi = {10.1016/S0079-7421(08)60536-8},
   issn = {00797421},
   issue = {C},
   journal = {Psychology of Learning and Motivation - Advances in Research and Theory},
   title = {Catastrophic Interference in Connectionist Networks: The Sequential Learning Problem},
   volume = {24},
   year = {1989},
}


@generic{French1999,
   abstract = {All natural cognitive systems, and, in particular, our own, gradually forget previously learned information. Plausible models of human cognition should therefore exhibit similar patterns of gradual forgetting of old information as new information is acquired. Only rarely does new learning in natural cognitive systems completely disrupt or erase previously learned information; that is, natural cognitive systems do not, in general, forget 'catastrophically'. Unfortunately, though, catastrophic forgetting does occur under certain circumstances in distributed connectionist networks. The very features that give these networks their remarkable abilities to generalize, to function in presence of degraded input, and so on, are found to be the root cause of catastrophic forgetting. The challenge in this field is to discover how to keep the advantages of distributed connectionist networks while avoiding the problem of catastrophic forgetting. In this article the causes, consequences and numerous solutions to the problem of catastrophic forgetting in neural networks are examined. The review will consider how the brain might have overcome this problem and will also explore the consequences of this solution for distributed connectionist networks.},
   author = {Robert M. French},
   doi = {10.1016/S1364-6613(99)01294-2},
   issn = {13646613},
   issue = {4},
   journal = {Trends in Cognitive Sciences},
   month = {4},
   pages = {128-135},
   pmid = {10322466},
   publisher = {Elsevier Current Trends},
   title = {Catastrophic forgetting in connectionist networks},
   volume = {3},
   year = {1999},
}


@article{Yann1998,
   abstract = {The MNIST database of handwritten digits, available from this page, has a training set of 60,000 examples, and a test set of 10,000 examples. It is a subset of a larger set available from NIST. The digits have been size-normalized and centered in a fixed-size image.\r\nIt is a good database for people who want to try learning techniques and pattern recognition methods on real-world data while spending minimal efforts on preprocessing and formatting.},
   author = {Lecun Yann and Cortes Corinna and Burges Christopher},
   journal = {The Courant Institute of Mathematical Sciences},
   title = {The MNIST database of handwritten digits},
   year = {1998},
}

@article{EWC,
   abstract = {The ability to learn tasks in a sequential fashion is crucial to the development of artificial intelligence. Until now neural networks have not been capable of this and it has been widely thought that catastrophic forgetting is an inevitable feature of connectionist models. We show that it is possible to overcome this limitation and train networks that can maintain expertise on tasks that they have not experienced for a long time. Our approach remembers old tasks by selectively slowing down learning on the weights important for those tasks. We demonstrate our approach is scalable and effective by solving a set of classification tasks based on a hand-written digit dataset and by learning several Atari 2600 games sequentially.},
   author = {James Kirkpatrick and Razvan Pascanu and Neil Rabinowitz and Joel Veness and Guillaume Desjardins and Andrei A. Rusu and Kieran Milan and John Quan and Tiago Ramalho and Agnieszka Grabska-Barwinska and Demis Hassabis and Claudia Clopath and Dharshan Kumaran and Raia Hadsell},
   doi = {10.1073/pnas.1611835114},
   issn = {10916490},
   issue = {13},
   journal = {Proceedings of the National Academy of Sciences of the United States of America},
   title = {Overcoming catastrophic forgetting in neural networks},
   volume = {114},
   year = {2017},
}

@article{Krizhevsky2009,
   abstract = {Groups at MIT and NYU have collected a dataset of millions of tiny colour images from the web. It is, in principle, an excellent dataset for unsupervised training of deep generative models, but previous researchers who have tried this have found it difficult to learn a good set of filters from the images. We show how to train a multi-layer generative model that learns to extract meaningful features which resemble those found in the human visual cortex. Using a novel parallelization algorithm to distribute the work among multiple machines connected on a network, we show how training such a model can be done in reasonable time. A second problematic aspect of the tiny images dataset is that there are no reliable class labels which makes it hard to use for object recognition experiments. We created two sets of reliable labels. The CIFAR-10 set has 6000 examples of each of 10 classes and the CIFAR-100 set has 600 examples of each of 100 non-overlapping classes. Using these labels, we show that object recognition is significantly improved by pre-training a layer of features on a large set of unlabeled tiny images.},
   author = {Alex Krizhevsky},
   doi = {10.1.1.222.9220},
   issn = {1098-6596},
   journal = {… Science Department, University of Toronto, Tech. …},
   title = {Learning Multiple Layers of Features from Tiny Images},
   year = {2009},
}


@inproceedings{SI,
   abstract = {While deep learning has led to remarkable advances across diverse applications, it struggles in domains where the data distribution changes over the course of learning. In stark contrast, biological neural networks continually adapt to changing domains, possibly by leveraging complex molecular machinery to solve many tasks simultaneously. In this study, we introduce intelligent synapses that bring some of this biological complexity into artificial neural networks. Each synapse accumulates task relevant information over time, and exploits this information to rapidly store new memories without forgetting old ones. We evaluate our approach on continual learning of classification tasks, and show that it dramatically reduces forgetting while maintaining computational efficiency.},
   author = {Friedemann Zenke and Ben Poole and Surya Ganguli},
   issn = {2640-3498},
   journal = {34th International Conference on Machine Learning, ICML 2017},
   title = {Continual learning through synaptic intelligence},
   volume = {8},
   year = {2017},
}



@inproceedings{MAS,
   abstract = {Humans can learn in a continuous manner. Old rarely utilized knowledge can be overwritten by new incoming information while important, frequently used knowledge is prevented from being erased. In artificial learning systems, lifelong learning so far has focused mainly on accumulating knowledge over tasks and overcoming catastrophic forgetting. In this paper, we argue that, given the limited model capacity and the unlimited new information to be learned, knowledge has to be preserved or erased selectively. Inspired by neuroplasticity, we propose a novel approach for lifelong learning, coined Memory Aware Synapses (MAS). It computes the importance of the parameters of a neural network in an unsupervised and online manner. Given a new sample which is fed to the network, MAS accumulates an importance measure for each parameter of the network, based on how sensitive the predicted output function is to a change in this parameter. When learning a new task, changes to important parameters can then be penalized, effectively preventing important knowledge related to previous tasks from being overwritten. Further, we show an interesting connection between a local version of our method and Hebb’s rule, which is a model for the learning process in the brain. We test our method on a sequence of object recognition tasks and on the challenging problem of learning an embedding for predicting <subject, predicate, object> triplets. We show state-of-the-art performance and, for the first time, the ability to adapt the importance of the parameters based on unlabeled data towards what the network needs (not) to forget, which may vary depending on test conditions.},
   author = {Rahaf Aljundi and Francesca Babiloni and Mohamed Elhoseiny and Marcus Rohrbach and Tinne Tuytelaars},
   doi = {10.1007/978-3-030-01219-9_9},
   issn = {16113349},
   journal = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
   title = {Memory Aware Synapses: Learning What (not) to Forget},
   volume = {11207 LNCS},
   year = {2018},
}


@inproceedings{iCaRL,
   abstract = {A major open problem on the road to artificial intelligence is the development of incrementally learning systems that learn about more and more concepts over time from a stream of data. In this work, we introduce a new training strategy, iCaRL, that allows learning in such a class-incremental way: only the training data for a small number of classes has to be present at the same time and new classes can be added progressively. iCaRL learns strong classifiers and a data representation simultaneously. This distinguishes it from earlier works that were fundamentally limited to fixed data representations and therefore incompatible with deep learning architectures. We show by experiments on CIFAR-100 and ImageNet ILSVRC 2012 data that iCaRL can learn many classes incrementally over a long period of time where other strategies quickly fail.},
   author = {Sylvestre Alvise Rebuffi and Alexander Kolesnikov and Georg Sperl and Christoph H. Lampert},
   doi = {10.1109/CVPR.2017.587},
   journal = {Proceedings - 30th IEEE Conference on Computer Vision and Pattern Recognition, CVPR 2017},
   title = {iCaRL: Incremental classifier and representation learning},
   volume = {2017-January},
   year = {2017},
}

@inproceedings{SelectiveER,
   abstract = {Deep reinforcement learning has emerged as a powerful tool for a variety of learning tasks, however deep nets typically exhibit forgetting when learning multiple tasks in sequence. To mitigate forgetting, we propose an experience replay process that augments the standard FIFO buffer and selectively stores experiences in a long-term memory. We explore four strategies for selecting which experiences will be stored: favoring surprise, favoring reward, matching the global training distribution, and maximizing coverage of the state space. We show that distribution matching successfully prevents catastrophic forgetting, and is consistently the best approach on all domains tested. While distribution matching has better and more consistent performance, we identify one case in which coverage maximization is beneficial - when tasks that receive less trained are more important. Overall, our results show that selective experience replay, when suitable selection algorithms are employed, can prevent catastrophic forgetting.},
   author = {David Isele and Akansel Cosgun},
   doi = {10.1609/aaai.v32i1.11595},
   issn = {2159-5399},
   journal = {32nd AAAI Conference on Artificial Intelligence, AAAI 2018},
   title = {Selective experience replay for lifelong learning},
   year = {2018},
}


@article{tinyER,
   abstract = {In continual learning (CL), an agent learns from a stream of tasks leveraging prior experience to transfer knowledge to future tasks. It is an ideal framework to decrease the amount of supervision in the existing learning algorithms. But for a successful knowledge transfer, the learner needs to remember how to perform previous tasks. One way to endow the learner the ability to perform tasks seen in the past is to store a small memory , dubbed episodic memory, that stores few examples from previous tasks and then to replay these examples when training for future tasks. In this work, we empirically analyze the effectiveness of a very small episodic memory in a CL setup where each training example is only seen once. Surprisingly, across four rather different supervised learning benchmarks adapted to CL, a very simple baseline, that jointly trains on both examples from the current task as well as examples stored in the episodic memory, significantly outperforms specifically designed CL approaches with and without episodic memory. Interestingly, we find that repetitive training on even tiny memories of past tasks does not harm generalization, on the contrary, it improves it, with gains between 7\% and 17\% when the memory is populated with a single example per class. Code is made available to reproduce the results.},
   author = {Arslan Chaudhry and Marcus Rohrbach and Mohamed Elhoseiny and Thalaiyasingam Ajanthan and Puneet K Dokania and Philip H S Torr and Marc ' Aurelio Ranzato},
   journal = {ICML},
   title = {Continual Learning with Tiny Episodic Memories},
   year = {2019},
}

@article{ProgressiveNet,
   abstract = {Learning to solve complex sequences of tasks--while both leveraging transfer and avoiding catastrophic forgetting--remains a key obstacle to achieving human-level intelligence. The progressive networks approach represents a step forward in this direction: they are immune to forgetting and can leverage prior knowledge via lateral connections to previously learned features. We evaluate this architecture extensively on a wide variety of reinforcement learning tasks (Atari and 3D maze games), and show that it outperforms common baselines based on pretraining and finetuning. Using a novel sensitivity measure, we demonstrate that transfer occurs at both low-level sensory and high-level control layers of the learned policy.},
   author = {Andrei A. Rusu and Neil C. Rabinowitz and Guillaume Desjardins and Hubert Soyer and James Kirkpatrick and Koray Kavukcuoglu and Razvan Pascanu and Raia Hadsell},
   doi = {10.48550/arxiv.1606.04671},
   month = {6},
   title = {Progressive Neural Networks},
   url = {http://arxiv.org/abs/1606.04671},
   year = {2016},
}

@article{PathNet,
   abstract = {For artificial general intelligence (AGI) it would be efficient if multiple users trained the same giant neural network, permitting parameter reuse, without catastrophic forgetting. PathNet is a first step in this direction. It is a neural network algorithm that uses agents embedded in the neural network whose task is to discover which parts of the network to re-use for new tasks. Agents are pathways (views) through the network which determine the subset of parameters that are used and updated by the forwards and backwards passes of the backpropogation algorithm. During learning, a tournament selection genetic algorithm is used to select pathways through the neural network for replication and mutation. Pathway fitness is the performance of that pathway measured according to a cost function. We demonstrate successful transfer learning; fixing the parameters along a path learned on task A and re-evolving a new population of paths for task B, allows task B to be learned faster than it could be learned from scratch or after fine-tuning. Paths evolved on task B re-use parts of the optimal path evolved on task A. Positive transfer was demonstrated for binary MNIST, CIFAR, and SVHN supervised learning classification tasks, and a set of Atari and Labyrinth reinforcement learning tasks, suggesting PathNets have general applicability for neural network training. Finally, PathNet also significantly improves the robustness to hyperparameter choices of a parallel asynchronous reinforcement learning algorithm (A3C).},
   author = {Chrisantha Fernando and Dylan Banarse and Charles Blundell and Yori Zwols and David Ha and Andrei A. Rusu and Alexander Pritzel and Daan Wierstra},
   doi = {10.48550/arxiv.1701.08734},
   month = {1},
   title = {PathNet: Evolution Channels Gradient Descent in Super Neural Networks},
   url = {http://arxiv.org/abs/1701.08734},
   year = {2017},
}

@inproceedings{HAT,
   abstract = {Catastrophic forgetting occurs when a neural network loses the information learned in a previous task after training on subsequent tasks. This problem remains a hurdle for artificial intelligence systems with sequential learning capabilities. In this paper, we propose a task-based hard attention mechanism that preserves previous tasks' information without affecting the current task's learning. A hard attention mask is learned concurrently to every task, through stochastic gradient descent, and previous masks are exploited to condition such learning. We show that the proposed mechanism is effective for reducing catastrophic forgetting, cutting current rates by 45 to 80%. We also show that it is robust to different hyperparameter choices, and that it offers a number of monitoring capabilities. The approach features the possibility to control both the stability and compactness of the learned knowledge, which we believe makes it also attractive for online learning or network compression applications.},
   author = {Joan Serra and Dídac Suris and Marius Mirón and Alexandras Karatzoglou},
   journal = {35th International Conference on Machine Learning, ICML 2018},
   title = {Overcoming Catastrophic forgetting with hard attention to the task},
   volume = {10},
   year = {2018},
}



@article{L2P,
   abstract = {The mainstream paradigm behind continual learning has been to adapt the model parameters to non-stationary data distributions, where catastrophic forgetting is the central challenge. Typical methods rely on a rehearsal buffer or known task identity at test time to retrieve learned knowledge and address forgetting, while this work presents a new paradigm for continual learning that aims to train a more succinct memory system without accessing task identity at test time. Our method learns to dynamically prompt (L2P) a pre-trained model to learn tasks sequentially under different task transitions. In our proposed framework, prompts are small learnable parameters, which are maintained in a memory space. The objective is to optimize prompts to instruct the model prediction and explicitly manage task-invariant and task-specific knowledge while maintaining model plasticity. We conduct comprehensive experiments under popular image classification benchmarks with different challenging continual learning settings, where L2P consistently outperforms prior state-of-the-art methods. Surprisingly, L2P achieves competitive results against rehearsal-based methods even without a rehearsal buffer and is directly applicable to challenging task-agnostic continual learning. Source code is available at https://github.com/google-research/l2p.},
   author = {Zifeng Wang and Zizhao Zhang and Chen-Yu Lee and Han Zhang and Ruoxi Sun and Xiaoqi Ren and Guolong Su and Vincent Perot and Jennifer Dy and Tomas Pfister},
   doi = {10.48550/arxiv.2112.08654},
   month = {12},
   title = {Learning to Prompt for Continual Learning},
   url = {http://arxiv.org/abs/2112.08654},
   year = {2021},
}

@inproceedings{Lopez2017,
   abstract = {One major obstacle towards AI is the poor ability of models to solve new problems quicker, and without forgetting previously acquired knowledge. To better understand this issue, we study the problem of continual learning, where the model observes, once and one by one, examples concerning a sequence of tasks. First, we propose a set of metrics to evaluate models learning over a continuum of data. These metrics characterize models not only by their test accuracy, but also in terms of their ability to transfer knowledge across tasks. Second, we propose a model for continual learning, called Gradient Episodic Memory (GEM) that alleviates forgetting, while allowing beneficial transfer of knowledge to previous tasks. Our experiments on variants of the MNIST and CIFAR-100 datasets demonstrate the strong performance of GEM when compared to the state-of-the-art.},
   author = {David Lopez-Paz and Marc'Aurelio Ranzato},
   issn = {10495258},
   journal = {Advances in Neural Information Processing Systems},
   title = {Gradient episodic memory for continual learning},
   volume = {2017-December},
   year = {2017},
}
 
@inproceedings{GR,
   abstract = {Attempts to train a comprehensive artificial intelligence capable of solving multiple tasks have been impeded by a chronic problem called catastrophic forgetting. Although simply replaying all previous data alleviates the problem, it requires large memory and even worse, often infeasible in real world applications where the access to past data is limited. Inspired by the generative nature of the hippocampus as a short-term memory system in primate brain, we propose the Deep Generative Replay, a novel framework with a cooperative dual model architecture consisting of a deep generative model ("generator") and a task solving model ("solver"). With only these two models, training data for previous tasks can easily be sampled and interleaved with those for a new task. We test our methods in several sequential learning settings involving image classification tasks.},
   author = {Hanul Shin and Jung Kwon Lee and Jaehong Kim and Jiwon Kim},
   issn = {10495258},
   journal = {Advances in Neural Information Processing Systems},
   title = {Continual learning with deep generative replay},
   volume = {2017-December},
   year = {2017},
}

@inproceedings{Rannen2017,
   abstract = {This paper introduces a new lifelong learning solution where a single model is trained for a sequence of tasks. The main challenge that vision systems face in this context is catastrophic forgetting: as they tend to adapt to the most recently seen task, they lose performance on the tasks that were learned previously. Our method aims at preserving the knowledge of the previous tasks while learning a new one by using autoencoders. For each task, an under-complete autoencoder is learned, capturing the features that are crucial for its achievement. When a new task is presented to the system, we prevent the reconstructions of the features with these autoencoders from changing, which has the effect of preserving the information on which the previous tasks are mainly relying. At the same time, the features are given space to adjust to the most recent environment as only their projection into a low dimension submanifold is controlled. The proposed system is evaluated on image classification tasks and shows a reduction of forgetting over the state-ofthe-art.},
   author = {Amal Rannen and Rahaf Aljundi and Matthew B. Blaschko and Tinne Tuytelaars},
   doi = {10.1109/ICCV.2017.148},
   issn = {15505499},
   journal = {Proceedings of the IEEE International Conference on Computer Vision},
   title = {Encoder Based Lifelong Learning},
   volume = {2017-October},
   year = {2017},
}

 @misc{sayce_2022,
 title={The number of tweets per day in 2022}, url={https://www.dsayce.com/social-media/tweets-day/}, journal={David Sayce}, publisher={Paper Gecko Ltd Paper Gecko Ltd. Publisher Logo},
 author={Sayce, David}, year={2022}, month={Aug}} 

@inproceedings{Cai2021,
   abstract = {Continual learning is the problem of learning and retaining knowledge through time over multiple tasks and environments. Research has primarily focused on the incremental classification setting, where new tasks/classes are added at discrete time intervals. Such an “offline” setting does not evaluate the ability of agents to learn effectively and efficiently, since an agent can perform multiple learning epochs without any time limitation when a task is added. We argue that “online” continual learning, where data is a single continuous stream without task boundaries, enables evaluating both information retention and online learning efficacy. In online continual learning, each incoming small batch of data is first used for testing and then added to the training set, making the problem truly online. Trained models are later evaluated on historical data to assess information retention. We introduce a new benchmark for online continual visual learning that exhibits large scale and natural distribution shifts. Through a large-scale analysis, we identify critical and previously unobserved phenomena of gradient-based optimization in continual learning, and propose effective strategies for improving gradient-based online continual learning with real data. The source code and dataset are available in: https://github.com/IntelLabs/continuallearning.},
   author = {Zhipeng Cai and Ozan Sener and Vladlen Koltun},
   doi = {10.1109/ICCV48922.2021.00817},
   issn = {15505499},
   journal = {Proceedings of the IEEE International Conference on Computer Vision},
   title = {Online Continual Learning with Natural Distribution Shifts: An Empirical Study with Visual Data},
   year = {2021},
}

@inproceedings{ACE,
   author = {Lucas Caccia and Rahaf Aljundi and Nader Asadi and Tinne Tuytelaars and Joelle Pineau and Eugene Belilovsky},
   journal = {International Conference on Learning Representations},
   title = {New Insights on Reducing Abrupt Representation Change in Online Continual Learning},
   url = {https://openreview.net/forum?id=N8MaByOzUfb},
   year = {2022},
}

@article{Van2019,
   abstract = {Standard artificial neural networks suffer from the well-known issue of catastrophic forgetting, making continual or lifelong learning difficult for machine learning. In recent years, numerous methods have been proposed for continual learning, but due to differences in evaluation protocols it is difficult to directly compare their performance. To enable more structured comparisons, we describe three continual learning scenarios based on whether at test time task identity is provided and--in case it is not--whether it must be inferred. Any sequence of well-defined tasks can be performed according to each scenario. Using the split and permuted MNIST task protocols, for each scenario we carry out an extensive comparison of recently proposed continual learning methods. We demonstrate substantial differences between the three scenarios in terms of difficulty and in terms of how efficient different methods are. In particular, when task identity must be inferred (i.e., class incremental learning), we find that regularization-based approaches (e.g., elastic weight consolidation) fail and that replaying representations of previous experiences seems required for solving this scenario.},
   author = {Gido M. van de Ven and Andreas S. Tolias},
   doi = {10.48550/arxiv.1904.07734},
   month = {4},
   title = {Three scenarios for continual learning},
   url = {http://arxiv.org/abs/1904.07734},
   year = {2019},
}

@inproceedings{ER,
   abstract = {Interacting with a complex world involves continual learning, in which tasks and data distributions change over time. A continual learning system should demonstrate both plasticity (acquisition of new knowledge) and stability (preservation of old knowledge). Catastrophic forgetting is the failure of stability, in which new experience overwrites previous experience. In the brain, replay of past experience is widely believed to reduce forgetting, yet it has been largely overlooked as a solution to forgetting in deep reinforcement learning. Here, we introduce CLEAR, a replay-based method that greatly reduces catastrophic forgetting in multi-task reinforcement learning. CLEAR leverages off-policy learning and behavioral cloning from replay to enhance stability, as well as on-policy learning to preserve plasticity. We show that CLEAR performs better than state-of-the-art deep learning techniques for mitigating forgetting, despite being significantly less complicated and not requiring any knowledge of the individual tasks being learned.},
   author = {David Rolnick and Arun Ahuja and Jonathan Schwarz and Timothy P. Lillicrap and Greg Wayne},
   issn = {10495258},
   journal = {Advances in Neural Information Processing Systems},
   title = {Experience replay for continual learning},
   volume = {32},
   year = {2019},
}


@article{Delange2021,
   abstract = {Artificial neural networks thrive in solving the classification problem for a particular rigid task, acquiring knowledge through generalized learning behaviour from a distinct training phase. The resulting network resembles a static entity of knowledge, with endeavours to extend this knowledge without targeting the original task resulting in a catastrophic forgetting. Continual learning shifts this paradigm towards networks that can continually accumulate knowledge over different tasks without the need to retrain from scratch. We focus on task incremental classification, where tasks arrive sequentially and are delineated by clear boundaries. Our main contributions concern: (1) a taxonomy and extensive overview of the state-of-the-art; (2) a novel framework to continually determine the stability-plasticity trade-off of the continual learner; (3) a comprehensive experimental comparison of 11 state-of-the-art continual learning methods; and (4) baselines. We empirically scrutinize method strengths and weaknesses on three benchmarks, considering Tiny Imagenet and large-scale unbalanced iNaturalist and a sequence of recognition datasets. We study the influence of model capacity, weight decay and dropout regularization, and the order in which the tasks are presented, and qualitatively compare methods in terms of required memory, computation time, and storage.},
   author = {Matthias De Lange and Rahaf Aljundi and Marc Masana and Sarah Parisot and Xu Jia and Ales Leonardis and Gregory Slabaugh and Tinne Tuytelaars},
   doi = {10.1109/TPAMI.2021.3057446},
   issn = {19393539},
   issue = {7},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   title = {A Continual Learning Survey: Defying Forgetting in Classification Tasks},
   volume = {44},
   year = {2021},
}

@generic{Parisi2019,
   abstract = {Humans and animals have the ability to continually acquire, fine-tune, and transfer knowledge and skills throughout their lifespan. This ability, referred to as lifelong learning, is mediated by a rich set of neurocognitive mechanisms that together contribute to the development and specialization of our sensorimotor skills as well as to long-term memory consolidation and retrieval. Consequently, lifelong learning capabilities are crucial for computational learning systems and autonomous agents interacting in the real world and processing continuous streams of information. However, lifelong learning remains a long-standing challenge for machine learning and neural network models since the continual acquisition of incrementally available information from non-stationary data distributions generally leads to catastrophic forgetting or interference. This limitation represents a major drawback for state-of-the-art deep neural network models that typically learn representations from stationary batches of training data, thus without accounting for situations in which information becomes incrementally available over time. In this review, we critically summarize the main challenges linked to lifelong learning for artificial learning systems and compare existing neural network approaches that alleviate, to different extents, catastrophic forgetting. Although significant advances have been made in domain-specific learning with neural networks, extensive research efforts are required for the development of robust lifelong learning on autonomous agents and robots. We discuss well-established and emerging research motivated by lifelong learning factors in biological systems such as structural plasticity, memory replay, curriculum and transfer learning, intrinsic motivation, and multisensory integration.},
   author = {German I. Parisi and Ronald Kemker and Jose L. Part and Christopher Kanan and Stefan Wermter},
   doi = {10.1016/j.neunet.2019.01.012},
   issn = {18792782},
   journal = {Neural Networks},
   title = {Continual lifelong learning with neural networks: A review},
   volume = {113},
   year = {2019},
}

@article{AljundiTaskFree,
   abstract = {Methods proposed in the literature towards continual deep learning typically operate in a task-based sequential learning setup. A sequence of tasks is learned, one at a time, with all data of current task available but not of previous or future tasks. Task boundaries and identities are known at all times. This setup, however, is rarely encountered in practical applications. Therefore we investigate how to transform continual learning to an online setup. We develop a system that keeps on learning over time in a streaming fashion, with data distributions gradually changing and without the notion of separate tasks. To this end, we build on the work on Memory Aware Synapses, and show how this method can be made online by providing a protocol to decide i) when to update the importance weights, ii) which data to use to update them, and iii) how to accumulate the importance weights at each update step. Experimental results show the validity of the approach in the context of two applications: (self-)supervised learning of a face recognition model by watching soap series and learning a robot to avoid collisions.},
   author = {Rahaf Aljundi and Klaas Kelchtermans and Tinne Tuytelaars},
   month = {12},
   title = {Task-Free Continual Learning},
   url = {http://arxiv.org/abs/1812.03596},
   year = {2018},
}


@article{Hu2020,
   abstract = {Continual learning systems will interact with humans, with each other, and
   with the physical world through time -- and continue to learn and adapt as they
   do. An important open problem for continual learning is a large-scale benchmark
   that enables realistic evaluation of algorithms. In this paper, we study a
   natural setting for continual learning on a massive scale. We introduce the
   problem of personalized online language learning (POLL), which involves fitting
   personalized language models to a population of users that evolves over time.
   To facilitate research on POLL, we collect massive datasets of Twitter posts.
   These datasets, Firehose10M and Firehose100M, comprise 100 million tweets,
   posted by one million users over six years. Enabled by the Firehose datasets,
   we present a rigorous evaluation of continual learning algorithms on an
   unprecedented scale. Based on this analysis, we develop a simple algorithm for
   continual gradient descent (ConGraD) that outperforms prior continual learning
   methods on the Firehose datasets as well as earlier benchmarks. Collectively,
   the POLL problem setting, the Firehose datasets, and the ConGraD algorithm
   enable a complete benchmark for reproducible research on web-scale continual
   learning.},
   author = {Hexiang Hu and Ozan Sener and Fei Sha and Vladlen Koltun},
   doi = {10.48550/arxiv.2007.09335},
   month = {7},
   title = {Drinking from a Firehose: Continual Learning with Web-scale Natural Language},
   url = {https://arxiv.org/abs/2007.09335},
   year = {2020},
}


@article{Shanahan2021,
   abstract = {We present an architecture that is effective for continual learning in an especially demanding setting, where task boundaries do not exist or are unknown, and where classes have to be learned online (with each example presented only once). To obtain good performance under these constraints, while mitigating catastrophic forgetting, we exploit recent advances in contrastive, self-supervised learning, allowing us to use a pre-trained, general purpose image encoder whose weights can be frozen, which precludes forgetting. The pre-trained encoder also greatly simplifies the downstream task of classification, which we solve with an ensemble of very simple classifiers. Collectively, the ensemble exhibits much better performance than any individual classifier, an effect which is amplified through specialisation and competitive selection. We assess the performance of the encoders-and-ensembles architecture on standard continual learning benchmarks, where it outperforms prior state-of-the-art by a large margin on the hardest problems, as well as in less familiar settings where the data distribution changes gradually or the classes are presented one at a time.},
   author = {Murray Shanahan and Christos Kaplanis and Jovana Mitrović},
   doi = {10.48550/arxiv.2105.13327},
   month = {5},
   title = {Encoders and Ensembles for Task-Free Continual Learning},
   url = {http://arxiv.org/abs/2105.13327},
   year = {2021},
}

@article{Jin2020,
   abstract = {Prior work on continual learning often operate in a “task-aware” manner, by assuming that the task boundaries and identifies of the data examples are known at all times. While in practice, it is rarely the case that such information are exposed to the methods (i.e., thus called “task-free”)–a setting that is relatively underexplored. Recent attempts on task-free continual learning build on previous memory replay methods and focus on developing memory construction and replay strategies such that model performance over previously seen examples can be best retained. In this paper, looking from a complementary angle, we propose a novel approach to “edit” memory examples so that the edited memory can better retain past performance when they are replayed. We use gradient updates to edit memory examples so that they are more likely to be “forgotten” in the future. Experiments on five benchmark datasets show the proposed method can be seamlessly combined with baselines to significantly improve the performance. Code has been released at https://github.com/INK-USC/GMED.},
   author = {Xisen Jin and Junyi Du and Xiang Ren},
   journal = {arXiv},
   title = {Gradient based memory editing for task-free continual learning},
   year = {2020},
}

@report{GDumb,
   abstract = {We discuss a general formulation for the Continual Learning (CL) problem for classification-a learning task where a stream provides samples to a learner and the goal of the learner, depending on the samples it receives, is to continually upgrade its knowledge about the old classes and learn new ones. Our formulation takes inspiration from the open-set recognition problem where test scenarios do not necessarily belong to the training distribution. We also discuss various quirks and assumptions encoded in recently proposed approaches for CL. We argue that some oversimplify the problem to an extent that leaves it with very little practical importance, and makes it extremely easy to perform well on. To validate this, we propose GDumb that (1) greedily stores samples in memory as they come and; (2) at test time, trains a model from scratch using samples only in the memory. We show that even though GDumb is not specifically designed for CL problems, it obtains state-of-the-art accuracies (often with large margins) in almost all the experiments when compared to a multitude of recently proposed algorithms. Surprisingly, it outperforms approaches in CL formulations for which they were specifically designed. This, we believe, raises concerns regarding our progress in CL for classification. Overall, we hope our formulation, characterizations and discussions will help in designing realistically useful CL algorithms, and GDumb will serve as a strong contender for the same.},
   author = {Ameya Prabhu and Philip H S Torr and Puneet K Dokania},
   title = {GDumb: A Simple Approach that Questions Our Progress in Continual Learning},
}


@article{Hsu2018,
   abstract = {Continual learning has received a great deal of attention recently with
   several approaches being proposed. However, evaluations involve a diverse set
   of scenarios making meaningful comparison difficult. This work provides a
   systematic categorization of the scenarios and evaluates them within a
   consistent framework including strong baselines and state-of-the-art methods.
   The results provide an understanding of the relative difficulty of the
   scenarios and that simple baselines (Adagrad, L2 regularization, and naive
   rehearsal strategies) can surprisingly achieve similar performance to current
   mainstream methods. We conclude with several suggestions for creating harder
   evaluation scenarios and future research directions. The code is available at
   https://github.com/GT-RIPL/Continual-Learning-Benchmark},
   author = {Yen-Chang Hsu and Yen-Cheng Liu and Anita Ramasamy and Zsolt Kira},
   doi = {10.48550/arxiv.1810.12488},
   month = {10},
   title = {Re-evaluating Continual Learning Scenarios: A Categorization and Case for Strong Baselines},
   url = {https://arxiv.org/abs/1810.12488},
   year = {2018},
}

@article{CLEAR,
   abstract = {Continual learning (CL) is widely regarded as crucial challenge for lifelong
AI. However, existing CL benchmarks, e.g. Permuted-MNIST and Split-CIFAR, make
use of artificial temporal variation and do not align with or generalize to the
real-world. In this paper, we introduce CLEAR, the first continual image
classification benchmark dataset with a natural temporal evolution of visual
concepts in the real world that spans a decade (2004-2014). We build CLEAR from
existing large-scale image collections (YFCC100M) through a novel and scalable
low-cost approach to visio-linguistic dataset curation. Our pipeline makes use
of pretrained vision-language models (e.g. CLIP) to interactively build labeled
datasets, which are further validated with crowd-sourcing to remove errors and
even inappropriate images (hidden in original YFCC100M). The major strength of
CLEAR over prior CL benchmarks is the smooth temporal evolution of visual
concepts with real-world imagery, including both high-quality labeled data
along with abundant unlabeled samples per time period for continual
semi-supervised learning. We find that a simple unsupervised pre-training step
can already boost state-of-the-art CL algorithms that only utilize
fully-supervised data. Our analysis also reveals that mainstream CL evaluation
protocols that train and test on iid data artificially inflate performance of
CL system. To address this, we propose novel "streaming" protocols for CL that
always test on the (near) future. Interestingly, streaming protocols (a) can
simplify dataset curation since today's testset can be repurposed for
tomorrow's trainset and (b) can produce more generalizable models with more
accurate estimates of performance since all labeled data from each time-period
is used for both training and testing (unlike classic iid train-test splits).},
   author = {Zhiqiu Lin and Jia Shi and Deepak Pathak and Deva Ramanan},
   doi = {10.48550/arxiv.2201.06289},
   month = {1},
   title = {The CLEAR Benchmark: Continual LEArning on Real-World Imagery},
   url = {https://arxiv.org/abs/2201.06289},
   year = {2022},
}

@article{Diaz2018,
   abstract = {Continual learning consists of algorithms that learn from a stream of
data/tasks continuously and adaptively thought time, enabling the incremental
development of ever more complex knowledge and skills. The lack of consensus in
evaluating continual learning algorithms and the almost exclusive focus on
forgetting motivate us to propose a more comprehensive set of implementation
independent metrics accounting for several factors we believe have practical
implications worth considering in the deployment of real AI systems that learn
continually: accuracy or performance over time, backward and forward knowledge
transfer, memory overhead as well as computational efficiency. Drawing
inspiration from the standard Multi-Attribute Value Theory (MAVT) we further
propose to fuse these metrics into a single score for ranking purposes and we
evaluate our proposal with five continual learning strategies on the iCIFAR-100
continual learning benchmark.},
   author = {Natalia Díaz-Rodríguez and Vincenzo Lomonaco and David Filliat and Davide Maltoni},
   doi = {10.48550/arxiv.1810.13166},
   month = {10},
   title = {Don't forget, there is more than forgetting: new metrics for Continual Learning},
   url = {https://arxiv.org/abs/1810.13166},
   year = {2018},
}


@inproceedings{RWalk,
   abstract = {Incremental learning (il) has received a lot of attention recently, however, the literature lacks a precise problem definition, proper evaluation settings, and metrics tailored specifically for the il problem. One of the main objectives of this work is to fill these gaps so as to provide a common ground for better understanding of il. The main challenge for an il algorithm is to update the classifier whilst preserving existing knowledge. We observe that, in addition to forgetting, a known issue while preserving knowledge, il also suffers from a problem we call intransigence, its inability to update knowledge. We introduce two metrics to quantify forgetting and intransigence that allow us to understand, analyse, and gain better insights into the behaviour of il algorithms. Furthermore, we present RWalk, a generalization of ewc++ (our efficient version of ewc [6]) and Path Integral [25] with a theoretically grounded KL-divergence based perspective. We provide a thorough analysis of various il algorithms on MNIST and CIFAR-100 datasets. In these experiments, RWalk obtains superior results in terms of accuracy, and also provides a better trade-off for forgetting and intransigence.},
   author = {Arslan Chaudhry and Puneet K. Dokania and Thalaiyasingam Ajanthan and Philip H.S. Torr},
   doi = {10.1007/978-3-030-01252-6_33},
   issn = {16113349},
   journal = {Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
   title = {Riemannian Walk for Incremental Learning: Understanding Forgetting and Intransigence},
   volume = {11215 LNCS},
   year = {2018},
}


@article{LwF,
   abstract = {When building a unified vision system or gradually adding new apabilities to a system, the usual assumption is that training data for all tasks is always available. However, as the number of tasks grows, storing and retraining on such data becomes infeasible. A new problem arises where we add new capabilities to a Convolutional Neural Network (CNN), but the training data for its existing capabilities are unavailable. We propose our Learning without Forgetting method, which uses only new task data to train the network while preserving the original capabilities. Our method performs favorably compared to commonly used feature extraction and fine-tuning adaption techniques and performs similarly to multitask learning that uses original task data we assume unavailable. A more surprising observation is that Learning without Forgetting may be able to replace fine-tuning with similar old and new task datasets for improved new task performance.},
   author = {Zhizhong Li and Derek Hoiem},
   doi = {10.1109/TPAMI.2017.2773081},
   issn = {19393539},
   issue = {12},
   journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
   title = {Learning without Forgetting},
   volume = {40},
   year = {2018},
}


@inproceedings{MIR,
   abstract = {Continual learning, the setting where a learning agent is faced with a never ending stream of data, continues to be a great challenge for modern machine learning systems. In particular the online or "single-pass through the data" setting has gained attention recently as a natural setting that is difficult to tackle. Methods based on replay, either generative or from a stored memory, have been shown to be effective approaches for continual learning, matching or exceeding the state of the art in a number of standard benchmarks. These approaches typically rely on randomly selecting samples from the replay memory or from a generative model, which is suboptimal. In this work we consider a controlled sampling of memories for replay. We retrieve the samples which are most interfered, i.e. whose prediction will be most negatively impacted by the foreseen parameters update. We show a formulation for this sampling criterion in both the generative replay and the experience replay setting, producing consistent gains in performance and greatly reduced forgetting.},
   author = {Rahaf Aljundi and Lucas Caccia and Eugene Belilovsky and Massimo Caccia and Min Lin and Laurent Charlin and Tinne Tuytelaars},
   issn = {10495258},
   journal = {Advances in Neural Information Processing Systems},
   title = {Online continual learning with maximally interfered retrieval},
   volume = {32},
   year = {2019},
}


@inproceedings{GSS,
   abstract = {A continual learning agent learns online with a non-stationary and never-ending stream of data. The key to such learning process is to overcome the catastrophic forgetting of previously seen data, which is a well known problem of neural networks. To prevent forgetting, a replay buffer is usually employed to store the previous data for the purpose of rehearsal. Previous works often depend on task boundary and i.i.d. assumptions to properly select samples for the replay buffer. In this work, we formulate sample selection as a constraint reduction problem based on the constrained optimization view of continual learning. The goal is to select a fixed subset of constraints that best approximate the feasible region defined by the original constraints. We show that it is equivalent to maximizing the diversity of samples in the replay buffer with parameters gradient as the feature. We further develop a greedy alternative that is cheap and efficient. The advantage of the proposed method is demonstrated by comparing to other alternatives under the continual learning setting. Further comparisons are made against state of the art methods that rely on task boundaries which show comparable or even better results for our method.},
   author = {Rahaf Aljundi and Min Lin and Baptiste Goujaud and Yoshua Bengio},
   issn = {10495258},
   journal = {Advances in Neural Information Processing Systems},
   title = {Gradient based sample selection for online continual learning},
   volume = {32},
   year = {2019},
}
@article{shalev2012online,
  title={Online learning and online convex optimization},
  author={Shalev-Shwartz, Shai and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={4},
  number={2},
  pages={107--194},
  year={2012},
  publisher={Now Publishers, Inc.}
}
